Conformal Prediction for Generative Models via Adaptive Cluster-Based Density Estimation

Conditional generative models map input variables to complex, high-dimensional distributions, enabling realistic sample generation in a diverse set of domains. A critical challenge with these models is the absence of calibrated uncertainty, which undermines trust in individual outputs for high-stakes applications. To address this issue, we propose a systematic conformal prediction approach tailored to conditional generative models, leveraging density estimation on model-generated samples. We introduce a novel method called CP4Gen, which utilizes clustering-based density estimation to construct prediction sets that are less sensitive to outliers, more interpretable, and of lower structural complexity than existing methods. Extensive experiments on synthetic datasets and real-world applications, including climate emulation tasks, demonstrate that CP4Gen consistently achieves superior performance in terms of prediction set volume and structural simplicity. Our approach offers practitioners a powerful tool for uncertainty estimation associated with conditional generative models, particularly in scenarios demanding rigorous and interpretable prediction sets.

==> Algorithms/CP4Gen_alg.tex <==
\begin{algorithm}[H]
\caption{CP4Gen: Conformal Prediction for Generative Models via $K$-means Clustering}
\label{alg:cp4gen}
\KwIn{Dataset $\textbf{D}=\{(X_i,Y_i)\}_{i=1}^N$, split into preliminary set $\textbf{D}_p$ and calibration set $\textbf{D}_c$; 
nominal level $\alpha$; 
ensemble size $M$; 
number of clusters $K$; 
nugget $\beta^2>0$.}
\KwOut{Predictive set $\widehat{C}_\alpha(X^\star)$ for a test covariate $X^\star$.}

\vspace{3mm}

\textbf{Step I: Fit Generative Model}\\
\Indp
Train a conditional generative model $q(Y|X)$ on $\textbf{D}_p$.\\
\Indm
\vspace{1mm}
\textbf{Step II: Compute Nonconformity Scores}\\
\Indp
\For{$(X_i,Y_i)\in\textbf{D}_c$}{
    \tcp{Draw an ensemble and cluster it}
    Sample $\hat{\textbf{Y}}_{i} = \{\hat{Y}_{i}^{1}, \dots, \hat{Y}_{i}^{M}\} \sim q(Y\!\mid\!X_i)$\;
    Run $K$-means on $\hat{\textbf{Y}}_{i}$\; 
    Obtain $K$ clusters, each with weight $w_{i}^{k}$, means $\boldsymbol{\mu}_{i}^{k}$, and covariances $\boldsymbol{\Sigma}_{i}^{k}$\;
    \tcp{Negative log mixture density score (with a small nugget)}
    \tcp{Mixture density approximated by its dominant component for easier prediction set inversion}
    $s_i \leftarrow -\log\!\left( \underset{1\leq k\leq K}{\max} w_{i}^{k}\,\mathcal{N}\!\big(Y_i;\,\boldsymbol{\mu}_{i}^{k},\,\boldsymbol{\Sigma}_{i}^{k}+\beta^2 I\big) \right)$.
}
Compute the $(1-\alpha)$ empirical quantile:
\[
Q_{1-\alpha} \;\leftarrow\; \mathrm{Quantile}_{1-\alpha}\big(\{s_i\}_{(X_i,Y_i)\in\textbf{D}_c}\cup\{\infty\}\big).
\]
\Indm
\textbf{Step III: Predictive set at test time}\\
\Indp
Sample $\hat{\textbf{Y}}_{\star} = \{\hat{Y}_{\star}^{1}, \dots, \hat{Y}_{\star}^{M}\} \sim q(Y\!\mid\!X^\star)$\;
Run $K$-means on $\hat{\textbf{Y}}_{\star}$ and obtain $\{w_{\star}^{k},\boldsymbol{\mu}_{\star}^{k},\boldsymbol{\Sigma}_{\star}^{k}\}_{k=1}^K$\;
Define the score at $Y$:
\[
s_\star(Y)\;=\;-\log\!\left(\underset{1\leq k\leq K}{\max} w_{\star}^{k}\,\mathcal{N}\!\big(Y;\,\boldsymbol{\mu}_{\star}^{k},\,\boldsymbol{\Sigma}_{\star}^{k}+\beta^2 I\big)\right);
\]

Return the prediction set:
\begin{align*}
\widehat{C}_\alpha(X^\star) 
& =\;\big\{Y:s_\star(Y)\le Q_{1-\alpha}\,\big\} \\
& = \bigcup_{k=1}^K \big\{Y:(Y-\boldsymbol{\mu}_{\star}^{k})^\top(\boldsymbol{\Sigma}_{\star}^{k}+\beta^2 I)^{-1}(Y-\boldsymbol{\mu}_{\star}^{k})\le r_k \big\},
\end{align*}
where $r_k$ is the threshold implied by $Q_{1-\alpha}$ for component $k$.

% \textit{(Efficient approximation)}: Replace the mixture by its maximal component to obtain a
% union of $K$ ellipsoids,
% \[
% \widehat{C}_\alpha(X^\star)\;\approx\;\bigcup_{k=1}^K
% \left\{\,y:\;(y-\mu_{\star k})^\top(\Sigma_{\star k}+\sigma^2 I)^{-1}(y-\mu_{\star k})\le r_k \right\},
% \]
% where $r_k$ is the threshold implied by $Q_{1-\alpha}$ for component $k$.
% \Indm

% \textbf{Notes}: $K$ trades off volume vs.\ structural complexity; setting $K\!=\!M$ recovers PCP as a special case.
\end{algorithm}
\begin{remark}
    In Algorithm \ref{alg:cp4gen}, we employ $K$-means to fit the Gaussian mixture model. It is worth noting that $K$-means relies on hard assignments, which can yield biased estimates of cluster means even with infinite data, particularly when the mixture components are not well separated \citep{jin2015}. As an alternative, the expectation maximization (EM) algorithm is a widely used approach for density estimation; however, it typically requires a larger computational budget for convergence, and may still be trapped in a local minima of estimation \citep{jin2016}. In experiments, we find that $K$-means produces clean and fast density fits across all tested datasets. An interesting future direction is to investigate more efficient yet accurate alternatives to $K$-means for mixture modeling.
\end{remark}

==> Sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. Yes
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. Yes
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes/No/Not Applicable]
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. Yes
    \item Complete proofs of all theoretical results. Yes
    \item Clear explanations of any assumptions. Yes  
  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). Yes
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). Yes
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). Yes
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). Yes
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. Not Applicable
    \item The license information of the assets, if applicable. Not Applicable
    \item New assets either in the supplemental material or as a URL, if applicable. Not Applicable
    \item Information about consent from data providers/curators. Not Applicable
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. Not Applicable
  \end{enumerate}

  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots. Not Applicable
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. Not Applicable
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. Not Applicable
  \end{enumerate}

\end{enumerate}

==> Sections/conclusion.tex <==
\section{Conclusion}

In this work, we proposed a general conformal prediction framework explicitly tailored for generative models.
Our general framework provides a critical missing piece in uncertainty quantification for generative modeling. 
It guides systematic design of conformal prediction sets with rigorous coverage guarantees from solely generated ensembles.
Within this framework, we derive a novel instantiation termed CP4Gen, 
which specifically mitigates sensitivity to outlier samples and reduces prediction set structural complexity, 
resulting in sets that are more interpretable and easier to use in downstream applications.
Through extensive evaluation on a range of synthetic and real-world datasets, 
including a climate precipitation emulation task, 
we demonstrated that CP4Gen consistently achieves valid empirical coverage close to the theoretical guarantees. 
Furthermore, CP4Gen significantly outperforms existing methods such as probabilistic conformal prediction (PCP) 
in terms of prediction set volume and structural complexity, 
substantiating its efficiency and practicality for real-world decision-making scenarios. 
In addition, CP4Gen constantly obtains superior performance on precipitation responses of varying dimensionality,
underscoring its scalability and effectiveness even when confronted with complex, high-dimensional distributions.
Overall, our general conformal prediction framework, with its CP4Gen instantiation, represents a meaningful advancement in the intersection of conformal prediction and generative modeling. 
It offers researchers and practitioners a powerful tool for calibrating uncertainty associated with generative models.
Future work could explore modifications to our framework to achieve guaranteed conditional coverage,
providing a new solution to rare event modeling.




% \begin{figure}
% \centering
%     \includegraphics[width=.32\linewidth]{image/fit_1.png}
%     \includegraphics[width=.32\linewidth]{image/fit_3.png}
%     \includegraphics[width=.32\linewidth]{image/fit_M.png}
% \caption{Fitting $q(Y|X)$ using different k in k-means algorithm}
% \label{fig:test}
% \end{figure}


% \subsection{High-dim output with Markov random field property}
% When the score is in high dimension, it is hard to compute a prediction set that covers all entries simultaneously, because this would lead to prediction which is 1) over-conservative; 2) lose marginal coverage because of correlation. However, most of the output in practice would have Markov random field, where every entry is only correlated with its neighborhood.

% For a generative model or single-output model, assume we could compute the joint prediction set for $Y^i$ and all its neighbors $\mathcal{N}_i$, denote it with $C_i$. Compute $C_i$ for $i=1,\dots, d_{y}$, and definite the prediction set
% \begin{align*}
%     C(X_{n+1}) &= \{Y\in\mathcal{Y}:Y_{\mathcal{N}_i}\in C_i, ~\forall~ i.\}
% \end{align*}
% This prediction set guarantees that we have marginal coverage over every neighborhood, and each prediction remains consistent.

==> Tables/Real_cont_metrics.tex <==
\begin{table}[!h]
    \caption{\textbf{CP Performance on Real World Datasets (Continued).} 
    Similar to Table \ref{tab:results:Real}, but for the additional datasets: Bio, Blog, Temperature, Bike, Taxi, and Energy.
    CP4Gen still outperforms PCP in terms of prediction set volume and structural complexity 
    while generally maintaining desired coverage rate of $90\%$ ($\alpha=0.1$).}
    \label{tab:results:Real_cont}
    \begin{center}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cccccccc}
        \toprule
        Metric & Method & Bio & Blog & Temperature & Bike & Taxi & Energy \\
        \midrule
        coverage & PCP & 0.90 & 0.91 & 0.90 & 0.90 & 0.90 & 0.95 \\
        coverage & CP4Gen & 0.90 & 0.91 & 0.90 & 0.90 & 0.90 & 0.94 \\
        \midrule
        complexity & PCP & 30.0 & 30.0 & 30.0 & 30.0 & 30.0 & 30.0 \\
        complexity & CP4Gen & 2.0 & 1.0 & 1.0 & 1.0 & 30.0 & 1.0 \\
        \midrule
        volume & PCP & 9.62 & 16.08 & 2.50 & 147.22 & 0.003 & 23.30 \\
        volume & CP4Gen & 8.94 & 13.84 & 2.23 & 120.93 & 0.003 & 21.83 \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}
